Seeing is not always believing: Benchmarking Human and Model Perception of AI-Generated Images

Photos serve as a way for humans to record what they experience in their daily lives, and they are often regarded as trustworthy sources of information. However, there is a growing concern that the advancement of artificial intelligence (AI) technology may produce fake photos, which can create confusion and diminish trust in photographs. This study aims to comprehensively evaluate agents for distinguishing state-of-the-art AI-generated visual content. Our study benchmarks both human capability and cutting-edge fake image detection AI algorithms, using a newly collected large-scale fake image dataset Fake2M. In our human perception evaluation, titled HPBench, we discovered that humans struggle significantly to distinguish real photos from AI-generated ones, with a misclassification rate of 38.7%. Along with this, we conduct the model capability of AI-Generated images detection evaluation MPBench and the top-performing model from MPBench achieves a 13% failure rate under the same setting used in the human evaluation. We hope that our study can raise awareness of the potential risks of AI-generated images and facilitate further research to prevent the spread of false information. More information can refer to https://github.com/Inf-imagine/Sentry.

==> Makefile <==
FIGURES_FOLDER := figures
PDFS := \
$(filter-out $(wildcard $(FIGURES_FOLDER)/*-crop.pdf),$(wildcard $(FIGURES_FOLDER)/*.pdf)) \
$(filter-out $(wildcard $(FIGURES_FOLDER)/**/*-crop.pdf),$(wildcard $(FIGURES_FOLDER)/**/*.pdf))
CROPPED_PDFS := $(PDFS:.pdf=-crop.pdf)

all: main.pdf

%.pdf: %.tex Makefile $(CROPPED_PDFS)
	pdflatex -synctex=1 -interaction=nonstopmode $<
	-bibtex $*.aux
	pdflatex -synctex=1 -interaction=nonstopmode $<
	pdflatex -synctex=1 -interaction=nonstopmode $<

.PHONY: figures
figures: $(CROPPED_PDFS)

.PRECIOUS: $(CROPPED_PDFS)
%-crop.pdf: %.pdf Makefile
	pdfcrop $<

.PHONY: clean upgrade
clean:
	find . -maxdepth 1 \
		\( -name "*.aux" -o -name "*.bbl" -o -name "*.blg" -o \
	           -name "*.log" -o -name "*.out" -o -name "*.pdf" -o \
		   -name "*.synctex.gz" \) | xargs $(RM)
	find $(FIGURES_FOLDER) -name "*-crop.pdf" | xargs $(RM)

YEAR := 2022

upgrade:
	curl https://media.neurips.cc/Conferences/NeurIPS$(YEAR)/Styles/neurips_$(YEAR).sty -o neurips.sty


==> checklist.tex <==
% \newpage
% \section*{Checklist}




% \begin{enumerate}


% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{See Section~\ref{sec:discussion}.}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{See Section~\ref{sec:discussion} for a brief discussion and Appendix~\maintoappref{sec:broader_impact} for the full discussion.}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}


% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerNA{}
%         \item Did you include complete proofs of all theoretical results?
%     \answerNA{}
% \end{enumerate}


% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerNo{The code and the data are proprietary.}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{See Section~\ref{sec:experiments} and Appendix~\maintoappref{app:extra_experiments_results}.}
%         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerNo{We do not observe large enough variance in our training runs to justify the computation cost incurred by multiple training runs. For the largest models, it is not feasible within our compute budget.}
%         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{Details can be found in Appendix~\maintoappref{app:large_scale_training}. In short, our largest run was trained on 1536 TPU chips for 15 days.}
% \end{enumerate}


% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators? \answerYes{We properly cited the prior methods on which our work is based, as well as prior datasets when appropriate (e.g., ALIGN).}
%   \item Did you mention the license of the assets? \answerNA{The assets we used are previous work for which we cited papers. We do mention the license of all visual assets we use for the figures of the paper in Appendix~\maintoappref{app:visual_content_credit}.}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerNo{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerYes{Our data was automatically scraped from million of webpages. See Datasheets~\cite{datasheet} in Appendix~\maintoappref{datasheets}.}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerYes{See Datasheets~\cite{datasheet} in Appendix~\maintoappref{datasheets}}.
% \end{enumerate}


% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}


% \end{enumerate}

==> content_version1/0_abstract.tex <==
\begin{quote}
\textit{Things are not always what they seem; the first appearance deceives many.}\\
% \qauthor{\textit{Phaedrus}}
\flushright{
\textit{Phaedrus}}
\end{quote}

\begin{abstract}

% Humans use photos to store information from daily visual observations. Truth, which is widely regarded as a cornerstone of our society, can be conveyed through photos. However, there is growing concern that emerging generative artificial intelligence could harm this social consensus by creating false and misleading information and damaging the social fabric. People urgently need to know if they can trust photos.
%Photos are used by humans to remember \xihui{remember->record} what they see in their daily lives and are often thought of as a reliable source of information.
%However, there is growing concern that emerging artificial intelligence technology could create fake images \xihui{images->photos}, which could cause confusion and damage trust in photos.
Photos serve as a way for humans to record what they experience in their daily lives, and they are often regarded as trustworthy sources of information. However, there is a growing concern that the advancement of artificial intelligence (AI) technology may produce fake photos, which can create confusion and diminish trust in photographs. % polished by chatgpt
%This study aimed to answer the question of whether the state-of-the-art Artificial Intelligence (AI) generation model could consistently trick human eyes and convey false facts. 
% To answer this question, we conducted a quantitative exploration of the ability of current state-of-the-art image generation models.
%With a high-quality quantitative study with fifty participants, we, for the first time, reveal that \textit{these models can significantly deceive human perception a significant degree (\textbf{38.7\%})}. 
% This study aims to answer the question of whether the current state-of-the-art AI-based visual content generation models can consistently deceive human eyes and convey false information. By conducting a high-quality quantitative study with fifty participants, we reveal, for the first time, that \textit{those generative models can significantly deceive human perception up to a significant degree (\textbf{38.7\%})}. 
This study aims to answer the question of whether the current state-of-the-art AI-based visual content generation models can consistently deceive human eyes and convey false information. By conducting a high-quality quantitative study with fifty participants, we reveal, for the first time, that \textit{humans cannot distinguish between real photos and AI-created fake photos to a significant degree \textbf{38.7\%}.}
% Done \xihui{human cannot distinguish between real photos and AI-created fake photos to a significant degree \textbf{38.7\%}.}
% Additionally, we found that an individual’s personal background, including gender, age, and AI background, does not significantly impact their ability to perceive AI-generated images. 
%We also discovered that an individual's personal background, such as their gender, age, and experience with AI-generated content (AIGC) , does not significantly affect their ability to detect AI-generated images.
Our study also finds that an individual's background, such as their gender, age, and experience with AI-generated content (AIGC), does not significantly affect their ability to distinguish AI-generated images from real photographs. 
% However, we did observe that AI-generated images are more likely to exhibit specific defects, which could potentially be used to improve human ability to distinguish between real and AI-generated images. This represents a potential direction for improving image generation models.
% \whlzy{logical}
%However, we did note that AI-generated images are more likely to have certain defects, which could help people distinguish between real and fake images. 
However, we do observe that there tend to be certain defects in AI-generated images that serve as cues for people to distinguish between real and fake photos.
% This observation also suggests a possible direction for improving image generation models.
% Finally, we reflect on the societal impacts of this recent technological leap and suggest potential directions for future research.
% We that this study can raise awareness of the potential risks of AI-generated images and encourage further research into improving image generation models to prevent the spread of false information. It is important for society to remain vigilant and develop strategies to counteract the potentially harmful effects of this technology.
%We hope that this study can raise awareness of the potential risks of AI-generated images and encourage further research into improving image generation models to prevent the spread of false information. 
%From a positive perspective, images generated by AI have the potential to revolutionize various industries and create a better future for humanity.
We hope that our study can raise awareness of the potential risks of AI-generated images and encourage further research to prevent the spread of false information. From a positive perspective, AI-generated images have the potential to revolutionize various industries and create a better future for humanity if they are used and regulated properly.

\end{abstract}

==> content_version1/1_intro.tex <==
\input{figure/fake_images}
\section{Introduction}



\input{figure/identify_real}

Photography, which captures images by recording light, has become an integral part of human society, serving as a vital medium for recording \textit{real} visual information. 
% following generated by ChatGPT
Its diverse applications range from documenting historical events and scientific discoveries to immortalizing personal memories and artistic expressions. 
% As a form of communication, photography transcends language barriers and enables people to connect with others across cultures and time, shaping our understanding of the world around us.
% following directly copied, should be modified ASAP
% https://photutorial.com/photos-statistics/#:~:text=There%20are%20about%2012.4%20trillion,10%E2%80%9314%25%20every%20year.
% There are about 12.4 trillion photos in the world, taking into account every photo taken since the first photo was taken by Joseph Nicéphore Niépce in 1826. According to the latest estimates, another 1.72 trillion photos are taken every year, so the total number increases by 10–14\% every year.
% Re-writed
Since the advent of photography with Joseph Nicéphore Niépce's first photograph of photographs in 1826, the global collection of photographs has expanded to an estimated 12.4 trillion photos. 
% Done Since the advent of photography with Joseph Nicéphore Niépce's first photograph in 1826, the global collection \xihui{the global collection of photographs?} has expanded to an estimated 12.4 trillion photos. 
This impressive number continues to rise with an annual increase of 1.72 trillion photos (10–14\% increasing rate every year)~\cite{photutorial}.

% 
In contrast to traditional photography, AI-driven image generation harnesses neural networks to learn synthesis rules from extensive image datasets, offering a novel approach for creating high-quality yet \textit{fake} visual content. By taking image descriptions or random noise as input, AI generates one or several images for users. Early methods employed GANs~\cite{Ian-2014-GAN, Andrew-2019-BigGAN, Han-2021-XMCGAN, Tero-2019-stylegan} as the generative architecture, while more recent diffusion-based techniques~\cite{Jonathan-2020-DDPM,Aditya-2022-DALLE2,Chitwan-2022-Imagen,Robin-2022-sd} have showcased improved diversity and generation quality. Therefore, AI-generated contents (AIGC) have gained popularity across various applications, such as AI-assisted design.

% Raise the question
Following the rapid advancements in AI-driven image generation algorithms, AI is now capable of producing a wide array of image styles, including those that closely resemble real photographs. 
At the Sony World Photography Awards in April 2023, the winner Eldagsen refused the award after revealing that his creation is made using AI.
Organizers of the award said that Eldagsen had misled them about the extent of AI that would be involved~\cite{bbc}.
Consequently, a critical question arises: \textit{Can humans distinguish whether an image is AI-generated?} This inquiry fundamentally questions the reliability of image information for conveying truth. Utilizing generated images to convey false information can have significant social repercussions, often misleading people about nonexistent events or propagating incorrect ideas, as shown in Fig.~\ref{fake images} and Fig.~\ref{identify}. A recent example involves the circulation of fake images depicting Trump's arrest~\cite{bbc2}, which garnered substantial social attention.

% To answer this question, ...
To address this question, we undertake a comprehensive study to assess the human ability in discerning AI-generated images. Specifically, we collect a dataset consisting of photo-style AI-generated images and real photographs sourced from the Internet. 
We then conduct a human evaluation involving participants from diverse backgrounds to determine their ability to distinguish real and fake images. 
Each participant is tasked with completing a test consisting of 100 randomized questions, where they must decide whether an image is real or generated by AI. 
If the participant deems an image to be fake, they are asked to provide a specific reason for their judgment.

Our primary finding establishes that \textit{state-of-the-art AI-generated images can indeed significantly deceive human perception.} According to our study, the average score for participants is 61.3\%, which indicates that they misclassified 38.7\% of the images, failing to accurately discern whether they are real or fake. 
Moreover, the highest score is only 73\%, illustrating that even the top-performing participant still misjudged 27\% of the images, while the lowest-scoring participant is only able to correctly identify 40\% of the images. % Done (whlzy) \bai{the lowest?}


Furthermore, our study reveals that \textit{humans are better at distinguishing AI-generated portrait images compared to other types of AI-generated images.} On the one hand, this observation suggests that the human eye is more adept at detecting defects in portrait images, where familiarity with human faces plays a critical role in assessing authenticity. 
On the other hand, it indicates that the current image generation models struggle with generating truly photo-realistic portraits.
% \xihui{This may also indicate the current AI models does not perform very well in generating photo-realistic portrait?}
% \whlzy{strange}
% 

Lastly, our results emphasize that \textit{an individual's background does not significantly impact their ability to perceive AI-generated images.} This insight implies that the ability to differentiate between real and fake images is not primarily determined by factors such as age and gender, underscoring the widespread challenge in detecting AIGC. 
Having technical knowledge, such as knowledge in generative AI, can only slightly enhance judgment (+2.7\%).

% Raise a conclusion
In this study, we demonstrate that state-of-the-art text-to-image synthesis techniques have the potential to deceive human perception. 
%On the one hand, rapid advancements in image synthesis enable individuals to create visually appealing images with quality nearing that of real photographs, facilitating the sharing of creative content. On the other hand, our findings uncover the possible risks associated with the use of AIGC for spreading false information and misleading viewers. This potential for misuse calls for more robust solutions in detecting fake images. Our work serves as a cautionary reminder to society regarding the implications of AIGC and the need for heightened awareness and vigilance.
While advancements in image synthesis have enabled individuals to create visually appealing images with quality approaching real photographs, our findings reveal the potential risks associated with using artificial intelligence-generated content (AIGC) for spreading false information and misleading viewers.
Our work highlights the need for more robust solutions in detecting fake images, as the potential for misuse of this technology is significant. We urge society to remain vigilant and aware of the implications of AIGC. Our study serves as a cautionary reminder of the risks associated with this technology and the need for heightened awareness and vigilance when using it.

==> content_version1/2_related.tex <==
% TODO: Refine

\section{Background}

\subsection{Image Generation}
% Generating a realistic image based on a given text description has proven to be a challenging task. 
% Initially, researchers heavily relied on GANs~\cite{Ian-2014-GAN,Andrew-2019-BigGAN,Han-2021-XMCGAN}, which were only effective within specific domains and datasets, assuming a closed-world environment. 
% However, with the advancement of diffusion models~\cite{Jonathan-2020-DDPM}, autoregressive transformers~\cite{vaswani-2017-transformer}, and large-scale language encoders~\cite{Colin-2020-T5,Tom-2020-GPT3,OpenAI-2023-GPT4,Alec-2021-CLIP}, the field of text-to-image synthesis has made remarkable progress towards an open-world with flexible text descriptions.
Generating photorealistic images based on given text descriptions has proven to be a challenging task. Previous GAN-based approaches~\cite{Ian-2014-GAN,Andrew-2019-BigGAN,Han-2021-XMCGAN,Tero-2019-stylegan} were only effective within specific domains and datasets, assuming a closed-world setting. However, with the advancements in diffusion models~\cite{Jonathan-2020-DDPM,yang-2021-score}, autoregressive transformers~\cite{vaswani-2017-transformer}, and large-scale language encoders~\cite{Colin-2020-T5,Tom-2020-GPT3,OpenAI-2023-GPT4,Alec-2021-CLIP}, significant progress has been made in high-quality photorealistic text-to-image synthesis with arbitrary text descriptions.
% \whlzy{openworld strange}

% Models such as DALL·E 2~\cite{Aditya-2022-DALLE2}, Imagen~\cite{Chitwan-2022-Imagen}, Stable Diffusion~\cite{Robin-2022-sd} and Midjourney~\cite{midjourney}, which are representative diffusion models, have demonstrated that producing photorealistic outputs is now possible with the aid of a pre-trained language encoder. 
% These models have surpassed GANs in both fidelity and diversity without the instability and mode collapse issues that GANs are prone to. 
% In addition to diffusion models, other models such as Make-A-Scene~\cite{Oran-2022-Make-A-Scene}, CogView~\cite{Ming-2021-CogView}, and Parti~\cite{Jiahui-2022-Parti} have also achieved amazing results in this field. 
% While these models exhibit unprecedented image synthesis ability, they require time-consuming iterative processes to achieve high-quality image sampling.
% Overall, the progress made in the field of text-to-image synthesis over the past few years is a testament to the potential of this technology.
State-of-the-art text-to-image synthesis approaches such as DALL·E 2~\cite{Aditya-2022-DALLE2}, Imagen~\cite{Chitwan-2022-Imagen}, Stable Diffusion~\cite{Robin-2022-sd}, and Midjourney~\cite{midjourney} have demonstrated the possibility of that generating high-quality, photorealistic images with diffusion-based generative models trained on large datasets. Those models have surpassed previous GAN-based models in both fidelity and diversity of generated images, without the instability and mode collapse issues that GANs are prone to.
In addition to diffusion models, other autoregressive models such as Make-A-Scene~\cite{Oran-2022-Make-A-Scene}, CogView~\cite{Ming-2021-CogView}, and Parti~\cite{Jiahui-2022-Parti} have also achieved amazing performance. While diffusion models and autoregressive models exhibit impressive image synthesis ability, they all require time-consuming iterative processes to achieve high-quality image sampling. 
% Done \xihui{Do we need to mention this? Readers may argue that sampling diffusion-based models are also time-consuming.}
However, the progress made in the field of text-to-image synthesis over the past few years is a testament to the potential of this technology.
% Despite the success achieved so far, the process of image generation in these models remains a challenging task, requiring a great deal of fine-tuning and tweaking to achieve the desired results. 

\subsection{Deepfake Generation and Detection}
% Done \whlzy{TODO(whlzy): Add https://www.mdpi.com/2076-3417/12/22/11312~\cite{Yanru-2022-HumanAI}}

% In December of 2017, a Reddit user going by the pseudonym "Deepfakes" shared pornographic videos that were created using open-source AI tools capable of swapping faces in images and videos. 
% Since then, the term "Deepfake" has been widely used to describe the generation of human appearances, particularly facial expressions, through AI methods. 
% The "Malicious Deep Fake Prohibition Act" of 2018 provides a definition of deepfake as videos and audios that have been realistically but falsely altered and are difficult to identify. 
% Similarly, the "DEEP FAKES Accountability Act" of 2019 defines deepfake as media that is capable of authentically depicting an individual who did not actually participate in the production of the content. 
% And ~\cite{Yisroel-2022-DeepfakeSurvey} defines deepfake as believable media generated by a deep neural network.
% In essence, deepfake~\cite{Chesney-2019-deepfake} refers to the creation of seemingly realistic but falsified images, audios, videos, and other digital media produced through AI methods, particularly deep learning.
In December 2017, a Reddit user going by the pseudonym "Deepfakes" shared pornographic videos created using open-source AI tools capable of swapping faces in images and videos. Since then, the term "Deepfake" has been widely used to describe the generation of human appearances, particularly facial expressions, through AI methods.
The "Malicious Deep Fake Prohibition Act" of 2018 provides a definition of deepfake as videos and audios that have been realistically but falsely altered and are difficult to identify. Similarly, the "DEEP FAKES Accountability Act" of 2019 defines deepfake as media that is capable of authentically depicting an individual who did not actually participate in the production of the content. Yisroel \textit{et al.}~\cite{Yisroel-2022-DeepfakeSurvey} defines deepfake as believable media generated by a deep neural network.
In essence, deepfake~\cite{Chesney-2019-deepfake} refers to the creation of seemingly realistic but falsified images, audios, videos, and other digital media produced through AI methods, particularly deep learning.

% Realistic deepfake media has posed a significant threat to privacy, democracy, national security, and society as a whole. These images and videos have the potential to bypass facial authentication, create political unrest, spread fake news, and even be used for blackmail. The proliferation of fake information through fabricated videos and images can severely undermine our trust in online digital content. Furthermore, the highly realistic nature of deepfake media makes it difficult for humans to identify them as being falsified. Thus, the ability to distinguish between deepfakes and real media has become an important, necessary, and urgent matter.
Realistic deepfake media has posed a significant threat to privacy, democracy, national security, and society as a whole. These images and videos have the potential to bypass facial authentication, create political unrest, spread fake news, and even be used for blackmail. The proliferation of fake information through fabricated videos and images can severely undermine our trust in online digital content.
Furthermore, the highly realistic nature of deepfake media makes it difficult for humans to identify them as being falsified. 
Thus, the ability to distinguish between deepfake and real media has become an important, necessary, and urgent matter.

In recent years, there have been many works~\cite{Xu-2019-detectfake,Sheng-2020-GeneratedFake} exploring how to distinguish whether an image is AI-generated. 
These works focus on images generated by GANs or small generation models~\cite{Ian-2014-GAN,Andrew-2019-BigGAN,Han-2021-XMCGAN,Tero-2019-stylegan}. 
Due to the limited quality of images generated by those methods, it is easy for humans to distinguish whether a photo is AI-generated or not. 
However, as the quality of generated images continues to improve with the advancement of recent generative models~\cite{Chitwan-2022-Imagen,midjourney,Robin-2022-sd,Aditya-2022-DALLE2}, it has become increasingly difficult for humans to identify whether an image is generated by AI or not. 
Lyu \textit{et al.}~\cite{Yanru-2022-HumanAI} provides an in-depth investigation into communication in human-AI co-creation, specifically focusing on the perceptual analysis of paintings generated by a text-to-image system.
Instead of exploring the human perception of AI-generated paintings, we study the human perception of AI-generated photographic images that may contain contradictions or absurdities that violate reality. Those AI-generated photorealistic images can potentially pose a significant threat to the accuracy of factual information.
In conclusion, the objective of our study is to investigate whether state-of-the-art AI-generated photographic images are capable of deceiving human perception.

% Done \bai{differences between this work and deepfack studies}



==> content_version1/3_setup.tex <==
% TODO: Refine (whlzy)
% Check ready



\section{Evaluation Setup}



% \subsection{Overview}
% Done \xihui{Maybe we can put this at the beginning of sec 3 and remove sec 3.1.}
% The question we aim to explore is whether humans can distinguish whether an image is generated by an AI model.
% We conduct an analysis of 50 sets of 100-question surveys to anwser this question.
Our objective is to investigate whether humans can distinguish if an image is AI-generated or not. 
We collect a set of AI-generated photorealistic images and real photographs, and conduct a human evaluation consisting of 50 sets of 100-question surveys on the collected images.
We describe the details of our data collection, human evaluation, and metrics for analyzing the results in the following subsections. 
%We conduct an analysis of 50 sets of 100-question surveys to answer this question.

\input{table/data_info}
\input{table/user_info}

\subsection{Data Collection}
% Now let us introduce the data collection process. 
% As it is difficult to determine whether arts or digital creations are generated by AI, we primarily collect photographic images across eight categories: humans, landscape, man, woman, record, plant, animal and object, as shown in Fig.~\ref{identify} and Tab.~\ref{data_info}.
% As it is difficult to determine whether arts or digital creations are generated by AI, we primarily collect photographic images across eight categories: humans, landscape, men, women, records, plants, animals, and objects, as shown in Fig.~\ref{identify} and Tab.~\ref{data_info}.
% As it is difficult to determine whether arts or digital creations are generated by AI, we primarily collect photographic images across eight categories: humans, landscapes, men, women, records, plants, animals, and objects, as shown in Fig.~\ref{identify} and Tab.~\ref{data_info}.
% 我们的数据分为两个部分，真的数据和假的数据
We collect photographic images across eight categories: \textit{Multiperson}, \textit{Landscape}, \textit{Man}, \textit{Woman}, \textit{Record}, \textit{Plant}, \textit{Animal}, and \textit{Object}, as shown in Fig.~\ref{identify} and Tab.~\ref{data_info}.
We collect a set of AI-generated images and a set of real photographs for each category.
%For each category, our data is divided into two parts: AI-generated images and real images.

\paragraph{Collecting AI-generated photorealistic images.}
% Initially, we appoint an annotation expert who read a substantial number of AI-generated images and real images. 
% He is able to discern to some extent whether a given image is generated by AI or is real.
% For our evaluation, we define low-quality AI-generated images as those with obvious visual defects that the annotator could easily identify as AI-generated images.
% And we define high-quality AI-generated images as those without any obvious visual defects that the annotator could not easily identify as AI-generated images.
% We utilize the state-of-the-art text-to-image AI generation models to create images of the aforementioned categories. 
% For each image, we employ diverse prompts to ensure maximum variation. 
% For some low-quality generated images, humans can easily perceive the visual defects in the image to determine whether it is AI-generated or not. 
% Therefore, we do not need to explore this issue in our evaluation. 
% We only focus on the high-quality AI-generated images.
% Finally, we employ the expertise of annotators to filter out low quality AI-generated images.
Firstly, we utilize Midjourney-V5~\cite{midjourney}, the state-of-the-art image generation model, to create photorealistic images of the aforementioned eight categories. 
For each category, we employ diverse prompts to ensure maximum variation. 
We use specialized prompt suffixes such as "normal color, aesthetic, shocking, very detailed, photographic, 8K, HDR" to improve the authenticity of the images.
%For some low-quality generated images, humans could easily perceive the visual defects in the image to determine whether it was AI-generated or not. 
% In real-world scenarios, people often use AI to generate images and strive to produce high-quality images without visual defects. 
We notice that in real-world scenarios, people use AI to generate images with the intention of creating high-quality images without visual defects, and users will select the best image from multiple generated images.
Therefore, we employ the expertise of annotators to filter out low-quality AI-generated images that can be easily determined as fake photos at the first glance.
% \xihui{Better to provide a ratio of filtered images, because how much data we filter out will affect the results. For example, if you pick the best image from 1000 generated images, the selected image will surely be a high-quality one which is indistinguishable from real photos.}
% we appoint an annotation expert to read a substantial number of AI-generated images and real images. 
% He is able to discern, to some extent, whether a given image was generated by AI or was real. 
% For our evaluation, we define low-quality AI-generated images as those with obvious visual defects that the annotator could easily identify as AI-generated images. We define high-quality AI-generated images as those without any obvious visual defects that the annotator could not easily identify as AI-generated images.
% We only focus on the high-quality AI-generated images. 
% \whlzy{这边介绍的有点口胡，怎么生成高质量的AI图像，只是说用了annotator去做了一下过滤，在prompt上有没有设计，怎么判断高质量低质量，这点要specify清楚}

% \whlzy{annotator,prompt,what is high quality?}

\paragraph{Collect real photos.}
We collect real photos from 500px~\cite{500px} and Google Images~\cite{google-images} by searching for photos with the same text prompts used for creating AI-generated images in the previous paragraph. The statistics of collected images in each category are shown in Tab.~\ref{data_info}.

% \input{table/metric_all_persons}

\subsection{Human Evaluation}
% Done \xihui{we can consider to swap the other of "human evaluation" and "data collection". It is more natural to first introduce the data collection and then introduce the human evaluation method.}
\paragraph{A high-quality fifty-participant human evaluation.}
% We recruit a total of 50 participants to complete our user study. 
% In order to ensure the comprehensiveness, fairness and quality of the experiment, we made efforts to ensure the diversity of the participants, as shown in Tab \ref{user_info}. Each participant will be required to complete a 100-question surveys without any time limit.
% It is worth noting that each participant completed the questionnaire with invigilator accompaniment to prevent random filling.
We recruit a total of 50 participants to participate in our human evaluation instead of using crowdsourcing. 
In order to ensure comprehensiveness, fairness, and quality of the evaluation, we make efforts to ensure the diversity of the participants, as shown in Tab.~\ref{user_info}. 
%Each participant completed the questionnaire in the presence of an invigilator to prevent random filling and to ensure the quality of the human evaluation results.
Each participant is asked to complete a questionnaire consisting of 100 questions without any time limit. 
%Each participant is required to carefully complete a 100-question survey without any time limit.
The questionnaires are completed in the presence of a project team member to guide the participant and ensure the quality of the human evaluation results.
% \whlzy{answer strange}
It is worth noting that we did not inform the participant about the ratio of real photos to AI-generated images in the questionnaires.

% Specifically, each question in the questionnaire provides the participant with an image, and the participant is asked to perform a binary classification to determine whether the image is generated by AI. 
% If the participant selects that the image is generated by AI, he/she will be required to choose one or more of the eight predefine judgment criteria options or provide their own judgment criteria, as shown in Tab.~\ref{judgement}.
% It is worth noting that each questionnaire consists of 50 real images and 50 AI-generated images, all of which are randomly sampled from the real image database and the AI-generated image database.
Specifically, each question in the questionnaire provides the participant with an image, and the participant is asked to determine whether the image is generated by AI or not. If the participant thinks that the image is generated by AI, he/she will be required to choose one or more reasons from the eight predefined judgment criteria options or provide their own judgment criteria. The eight options are explained below:

\noindent{\textbf{$\bullet$}} Detail: AI-generated images may lack fine details, such as wrinkles in clothing or hair details.
% "Detail problem" refer to situations where some details in AI-generated images are not realistic or unreasonable, such as wrinkles in clothing or hair details. 

\noindent{\textbf{$\bullet$}} Smooth: AI-generated images may appear smoother or more uniform than real photos, such as smooth skin or unrealistic facial expressions.
% "Smoothing problem" refer to situations where AI-generated images have overly smooth skin, resulting in unrealistic facial expressions and features.

\noindent{\textbf{$\bullet$}} Blur: AI-generated images may be blurry, such as blurry or unclear edges.
% "Blur problem" refer to situations where AI-generated images are blurry or unclear, resulting in obvious artifact.

\noindent{\textbf{$\bullet$}} Color: AI-generated images may have unrealistic or inconsistent colors, such as colors that are too bright, too dark, or like the color of animation.
% "Color problem" refer to situations where the colors in AI-generated images are not realistic or coordinated, such as colors that are too bright, too dark or like the color of animation. 

\noindent{\textbf{$\bullet$}} Shadow \& Light: AI-generated images may have unrealistic or inconsistent shadows and lighting, such as shadows or lightning that violate physics.
%  "Shadow&Light problem" refer to situations where the position and shape of light sources and shadows in AI-generated images are unreasonable, resulting in unnatural lighting effects. 

\noindent{\textbf{$\bullet$}} Daub: AI-generated images may contain rough, uneven, or poorly applied colors or textures.
% efer to situations where AI-generated images have been excessively daubed, resulting in lost details or unrealistic images

\noindent{\textbf{$\bullet$}} Rationality: AI-generated images may contain irrational/illogical/contradictory contents.
% between objects refer to situations where the relationship between objects in AI-generated images is not reasonable, such as incorrect size proportions or unreasonable positions.

\noindent{\textbf{$\bullet$}} \textcolor{MyDarkgray}{Intuition}: people may judge whether a photo is AI-generated or not by intuition and cannot describe the exact reasons.



%, as shown in Tab.~\ref{judgement}.
It is important to point out that each questionnaire consists of 50 real images and 50 AI-generated images, all of which are randomly sampled from the real image database containing 244 images and the AI-generated image database containing 151 images.

% Done (whlzy) \bai{describe the protocol more clearly and justify the protocol: not know the ratio of real and fack; does not control the time; not required to answer the question; not using crowdsourcing}

\paragraph{Why not crowdsourcing human evaluation?}
% Inspired by ~\cite{Robert-2021-humanvsmachine}, we aim to collect high-quality human evaluation data instead of noisy crowdsourcing data.
% Our human evaluation with a limited number of subjects in a controlled environment, and conducting multiple experiments, is commonly referred to as the "small-N design".
% As the title of the article "Small is beautiful: In defense of the small-N design"~\cite{Smith-2018-small}, "small-N design" is the core of high-quality psychophysics.
% The "crowdsourcing" involves many observers in a uncontrollable noisy setting, each performing fewer trials. 
% In contrast, we strive to ensure that each participant with diverse background takes the full 100-question surveys in a quiet, relaxed, controllable, and invigilator-monitored environment.
% These factors contribute to high data quality.
Inspired by Robert \textit{et al.}~\cite{Robert-2021-humanvsmachine}, we aim to collect high-quality human evaluation data instead of noisy crowdsourcing data to ensure the high quality of the results. Our human evaluation, with a limited number of participants in a controlled environment, and conducting multiple experiments, is commonly referred to as the ``small-N design''. As the article "Small is beautiful: In defense of the small-N design" \cite{Smith-2018-small} suggests, the "small-N design" is the core of high-quality psychophysics. Crowdsourcing involves many participants in an uncontrollable, noisy setting, with each performing fewer trials. In contrast, we strive to ensure that each participant, with diverse backgrounds, takes the full 100-question survey in a quiet, relaxed, controllable, and monitored environment. Those factors contribute to high data quality.



\input{table/metric_all_persons}
\subsection{Metrics}
% Here, we primarily employ four commonly evaluation metrics to analyze our problem and highlight their respective meanings in the context of our problem.
% We define positive samples as AI-generated images and negative samples as real images for our problem.
% Now we can calculate \textit{Accuracy}, \textit{Precision}, \textit{Recall}, and \textit{False Omission Rate} in our problem context, as shown in Tab.~\ref{metric_all_persons}.
We employ four commonly used evaluation metrics to analyze our results and highlight their respective meanings in the context of our problem. We define positive samples as AI-generated images and negative samples as real images for our problem, and then calculate Accuracy, Precision, Recall, and False Omission Rate (FOR) in the context of our problem, as shown in Tab.~\ref{metric_all_persons}.

% \paragraph{Accuracy}
\textbf{Accuracy}
% Accuracy is used as a statistical measure of how well a binary classification test correctly identifies or excludes a condition. 
% In our problem, accuracy represents the average precision of humans.
is a statistical measure used to evaluate how well a binary classification test correctly identifies or excludes a condition. In our study, accuracy represents the average precision of humans in distinguishing AI-generated images from real images.

% \paragraph{Precision}
\textbf{Precision}
% Precision is the percentage of predicted positive cases that are actually positive. 
% In our problem, high precision represents that humans are good at identifying the AI-generated images and do not misclassify real images as AI-generated images.
is the percentage of predicted positive cases that are actually positive. In our study, high precision represents the proportion of AI-generated images out of the total number of images that are predicted as AI-generated ones. %that humans are good at identifying AI-generated images and do not misclassify real images as AI-generated images.

% \paragraph{Recall}
\textbf{Recall}
% Recall is the percentage of true positive cases that are actually predicted as positive. 
% In our problem, recall represents the proportion of images correctly identified as AI-generated images out of the total number of AI-generated images.
is the percentage of true positive cases that are actually predicted as positive. In our study, recall represents the proportion of AI-generated images that are correctly identified as such out of the total number of AI-generated images.



% \paragraph{FOR}
\textbf{FOR}
% False omission rate (FOR) is the percentage of false negatives out of all negative cases.
% In our problem, FOR represents the proportion of AI-generated images identified as real images out of the total number of the images.
is the percentage of false negatives out of all negative cases. In our problem, FOR represents the proportion of real images misidentified as AI-generated images out of the total number of images.

% \paragraph{$F_{1}$ Score}
% $F_{1}$ Score is 



==> content_version1/4_eval.tex <==

\input{figure/all_categories_with_all_persons}
\section{Human Evaluation Findings and Analysis}

% \whlzy{Add a overview here.}
% \whlzy{For each problem, give a fast answer}

\subsection{Overall Ability to Distinguish Real and AI-generated Images}

\paragraph{Results.}
% The overall results are shown in Figure~\ref{all categories with all persons}. According to our study, participants are able to successfully judge 61.3\% of images, which means that 38.7\% images are incorrectly be regarded as real or fake images. Even the participant with highest score can only reach 78\%, and the participant with the lowest score reach around 40\%. Such a observation shows that people can easily be tricked by the mixture of real and AI-generated fake images. Besides, the results show that for real images from Internet, human has a average chance of 66.9\% to correctly sort them as true images; while for AI-generated images, people are more likely to mis-guieded and sort them as true with a possibility of 44.2\%. 
The results are shown in Fig.~\ref{all categories with all persons}. Our study indicates that participants on average are able to correctly distinguish 61.3\% of the images, while 38.7\% of the images were misclassified. The highest-performing participant is able to correctly distinguish 73\% of the images, while the lowest-performing participant is only able to correctly distinguish 40\% of the images. These observations demonstrate that a combination of real and AI-generated fake images can easily deceive people. Moreover, the results reveal that humans have an average probability of 66.9\% of correctly identifying real photos from the internet, whereas for AI-generated images, people are more likely to be misled and incorrectly identify them as real with an average probability of 44.2\%.
% 39% of all images are missed by people and are actually generated by AI.

% X\% ..., Y\% ...? (Give some illustration about the figure.)

\paragraph{Analysis.}
% An interesting observation we see from the above data is that even for the real images collected from Internet, participants are still only able to correctly distinguish 66.9\% images, which supposed should be correctly sort out by 100\%. This observation shows that the AI-generated not only convey wrong information towards human, but also make the true information much harder to be trusted. Another interesting conclusion is that human do have better distinguish ability for real-images, thanks to the all life training for seeing the real images. However, the gap between real images perception and AI-generated images is only 11.1\%, future generative AI models have the potential to quickly solve this gap. 
An intriguing observation from the above data is that even for real images collected from the Internet, participants were only able to correctly identify 66.9\% of the images that should have been correctly sorted out 100\% of the time. This finding demonstrates that AI-generated images not only convey incorrect information to humans but also erode people's trust in accurate information. 
Additionally, our study reveals that humans possess a superior ability to identify real photos than fake photos, which can be attributed to their lifetime experience.
Despite this, the difference between real image perception and AI-generated image perception is only 11.1\%, and we believe that future generative AI models could further narrow this gap.



% \noindent\textcolor{MyDarkBlue}{\textbf{$\bullet$\quad A :}}
% \paragraph{Most people will be cheated by XXX.}
% \paragraph{Only a few can consistently find out the AIGC images.}
% \subsection{Distinguish Abilities of participants with Different Genders.}
% \paragraph{Data}
% \paragraph{Analysis}
% \
% \noindent\textcolor{MyDarkBlue}{\textbf{$\bullet$\quad A :}}
% \input{figure/all categories with man and woman}
% \paragraph{Portrait images is easier to distinguish.}
% \paragraph{XXX is difficult to ..}

% \subsection{Distinguish Abilities of participants with and without Played-AIGC Background}
\subsection{Distinguishing Abilities of Participants with Various Personal Backgrounds}
\paragraph{Results.}
\input{figure/all_categories_with_people_have_played_with_AIGC_and_have_not_played_with_AIGC}
% We also evaluate whether personal AI background affects the distinguish ability. As shown in Figure~\ref{all categories with people have played with AIGC and have not played with AIGC}, people with AIGC background, gets a better score (+2.7\%). Specifically, for real images, AIGC background helps little (+0.7\%), while participants with AIGC background gain much better results (+3.7\%) for AI-generated images. Also, results from AIGC background participants have lower variance. 
We explored the effect of an individual's AIGC background (AIGC background specifically refers to participants who have played with AIGC) on their ability to distinguish. In Fig.~\ref{all categories with people have played with AIGC and have not played with AIGC}, we can see that individuals who have played with AIGC scored slightly better than those without AIGC background (+2.7\%). Interestingly, their AIGC background seemed to have only slight effects on their ability to identify real images, with only a slight increase of 0.7\%. However, when it came to AI-generated images, participants with an AIGC background performed significantly better, with a boost of 3.7\% in their results. Furthermore, we observed that individuals with AIGC background demonstrated less variation in their scores, suggesting a more consistent ability to distinguish between real and AI-generated images.
We also observed that gender has little impact on the human ability to distinguish, as outlined in the Appendix.

\paragraph{Analysis.}
% Playing with generative models do improve the distinguish ability of participants. This improvement mainly comes from better find out which images are more likely to be fake and generated by AI. 
Our thorough research and analysis demonstrate that a person's knowledge and experience with AIGC do not play a significant role in their ability to distinguish between real and AI-generated images. 
Specifically, when it comes to AI-generated images, participants who have played with AIGC have a slightly improved ability to distinguish between the two categories. 
This is mainly due to their enhanced skills in identifying which images are more likely to be fake or generated by AI. 
Furthermore, this suggests that additional training and exposure to generative models may be beneficial for individuals by helping them make more informed decisions and avoid any potential misinformation or confusion that may arise from misinterpreting images.

% \noindent\textcolor{MyDarkBlue}{\textbf{$\bullet$\quad A :}}
% \subsection{Analyse the Failure Cases}
% \paragraph{Data}
\input{figure/All_images_with_different_categories_for_all_persons}
\subsection{Distinguishability of different photo categories}
\paragraph{Results.}
% This study also evaluate the human distinguish ability across different photo category, shown in Figure~\ref{All images with different categories for all persons} and Table~\ref{metric_all_persons}. For different category, participants show dramatically different distinguish ability. For example, participants can distinguish `Human' with a ratio of 67.5\% while only able to correctly judge `Object' with a ratio of 50.8\%. There is a gap of 16.7\% between the easiest category and hardest category. 
%In this study, we aimed to investigate the accuracy of human perception in discerning between different photo categories. 
We aim to investigate the difficulties for humans to distinguish real and fake images of different image categories.
The results were presented in Fig.~\ref{All images with different categories for all persons} and Tab.~\ref{metric_all_persons}. It is observed that the participants had varying ability levels in distinguishing real or fake images from different categories. For instance, the participants can distinguish real or fake images from the category \textit{Multiperson} with a relatively high accuracy rate of 67.5\%, whereas they can only correctly distinguish real or fake from the category \textit{Object} with a much lower accuracy rate of 50.8\%. Our results indicate a significant 16.7\% difference between the accuracy rates of the easiest and most challenging categories. These findings suggest that there may be significant differences in the way humans perceive different photo categories, which could have important implications for further research in this area.
It also indicates that the current AI-based generative models may be good at generating some categories but not so good at generating other categories.
% \xihui{It also indicates that the current AI-based generative models may be good at generating some categories but not so good at generating other categories.}

\paragraph{Analysis.}
% Above data show that current generative AI do have areas of expertise and areas of weakness. In this study, we find current state-of-the-art AI image generation model can generate `Object' in an incredibly realistic level, easy to trick human eyes. On the other side, AI-generated human images is much easier to be detected by human. As shown in the Table~\ref{metric_all_persons}, participants distinguish `Human' `Man' and `Women' easier than other category. One potential reason is human brain is better at distinguish human images.
The presented data offers valuable insights into the strengths and limitations of generative AI. The study indicates that current state-of-the-art AI image generation models excel in creating \textit{Object} images that are incredibly realistic, often even fooling the human eye. However, AI still struggles when it comes to generating human images. As shown in Tab.~\ref{metric_all_persons}, participants found it considerably easier to distinguish real or fake images from \textit{Multiperson}, \textit{Man}, and \textit{Woman} categories when compared to other categories. This phenomenon could be attributed to the fact that the human brain is more sensitive to images of humans, which is an essential aspect of our cognitive processing.
% Furthermore, this study has opened up new avenues for research into generative AI, and it presents exciting possibilities for future developments in this field. 
% By identifying the limitations of current image generation models, researchers can now focus on overcoming these challenges and developing more advanced AI systems. This could lead to a wide range of applications, from more realistic video game characters to highly accurate medical imaging.
% Overall, this study highlights the importance of continued research and development in the field of generative AI. While there are still significant challenges to overcome, the potential benefits of this technology are vast, and it is clear that AI will play an increasingly important role in our lives in the years to come.

\subsection{Results of the Judgment Criteria and Analysis of the AIGC Defects}

\input{table/judgement}
\input{figure/AIGC_defect}

% We predefine eight judgment criteria options based on our experience, including "Detail problem", "Smooth problem", "Intuition", "Blur problem", "Color problem", "Shadow\&Light problem", "Daub problem", and "Rationality problem". 
% If participants' judgment criteria do not belong to these eight categories, they can input their own judgment criteria. 
% The specific statistics of judgment criteria for correctly selecting the AI-generated images are shown in the Tab.~\ref{judgement}.
% There are many criteria for each judgment category, and these results indicate that even high-quality AI-generated images still have various defects.
% The most common issues are "Detail problem" and "Smooth problem".
% It indicates that the current state-of-the-art image generation model has poor ability to generate fine details and often produce over-smoothing portraits.
% The proportion of participants who chose "intuition" is about 14\%, indicating that it is difficult for people to describe obvious defects in AI-generated images and they have to rely on their feelings to make a judgment.
\paragraph{Results.}
We predefined eight judgment criteria options based on our experience, including "Detail problem", "Smooth problem", "Blur problem", "Color problem", "Shadow \& Light problem", "Daub problem", "Rationality problem", and "\noindent\textcolor{MyDarkgray}{Intuition}".
% If participants' judgment criteria does not belong to these eight categories, they could input their own judgment criteria.
The specific statistics of judgment criteria for correctly selecting the AI-generated images are shown in Tab.~\ref{judgement}.
% There are many criteria for each judgment category, and 
These results indicate that even high-quality AI-generated images still have various defects.
The most common issues are "Detail problem" and "Smooth problem" with a high rate of 28\% and 17\%, respectively.
It indicates that the current state-of-the-art image generation model has a poor ability to generate fine details and often produces over-smoothed portraits.
It is worth noting that the proportion of participants who choose "\noindent\textcolor{MyDarkgray}{Intuition}" is about \noindent\textcolor{MyDarkgray}{14\%}, indicating that it is difficult for people to describe obvious defects in AI-generated images, even if they can successfully identify the AI-generated images.
% They have to rely on their intuition to make a judgment.

\paragraph{Analysis.}
Based on the user data we collected above, we summarize and show nine shortcomings of the current AIGC, as shown in Fig.~\ref{AIGC defects}:
(1) "Hand problem" refers to situations where fingers overlap or have unreasonable shapes (multi fingers), resulting in images that are not realistic.
(2) "Smoothing problem" refers to situations where AI-generated images have overly smooth skin, resulting in unrealistic facial expressions and features.
(3) "Shadow\&Light problem" refers to situations where the position and shape of light sources and shadows in AI-generated images are unreasonable, resulting in unnatural lighting effects.
(4) "Character problem" refers to situations where incorrect signs and texts appear in AI-generated images, which do not match reality.
(5) "Detail problem" refers to situations where some details in AI-generated images are not realistic or unreasonable, such as wrinkles in clothing or hair details.
(6) "Blur problem" refers to situations where AI-generated images are blurry or unclear, resulting in obvious artifacts.
(7) "Color problem" refers to situations where the colors in AI-generated images are not realistic or coordinated, such as colors that are too bright, too dark, or like the color of animation.
(8) "Daub problem" refers to situations where AI-generated images have been excessively daubed, resulting in lost details or unrealistic images.
(9) "Rationality problem" between objects refers to situations where the relationship between objects in AI-generated images is not reasonable, such as incorrect size proportions or unreasonable positions.



==> content_version1/5_discuss.tex <==
% TODO: Refine (whlzy)
% Finish (whlzy)

\section{Discussion, Broader Impact and Conclusion}

% \whlzy{For each problem, give a fast answer}

\subsection{Discussion}

\paragraph{Can AIGC deceive humans now?}
% With the rapid advancements in AI-driven image generation, AI is now capable of producing highly realistic images that can deceive human perception. 
% Despite the fact that humans can sometimes discern low-quality AI-generated images, high-quality deepfake images are becoming increasingly difficult to distinguish from real ones. 
% At the Sony World Photography Awards in April 2023, the winner Eldagsen refused his award after revealing that his creation was made using AI and organisers of the award said that Eldagsen had mis-led them about the extent of AI that would be involved~\cite{bbc}.
% % We can no longer judge whether an image is generated by AI based on the quality of the image. Instead, we need to assess the validity of AI-generated images based on whether the objects are too perfect, their consistency with other objects, and whether they violate physical laws.
% Our human evaluation results indicate that the state-of-the-art models can significantly deceive human perception a significant degree (38.7\%).
% For humans, it is no longer possible to judge whether an image is generated by AI based solely on image quality. Instead, we need to consider factors such as whether the portrait is too smooth, the coherence and consistency between objects, and whether there are any violations of physical laws in the image.
With the recent rapid advancements in generative AI, AI is now capable of producing highly photorealistic images with rich backgrounds, vivid characters, and beautiful lighting.
% that can deceive human perception. 
% Despite the fact that humans can sometimes discern low-quality AI-generated images, high-quality AI-generated images are becoming increasingly difficult to distinguish from real ones. 
Although people may able to occasionally differentiate low-quality AI-generated images, it is becoming more and more difficult to distinguish high-quality AI-generated images from real photography.
% At the Sony World Photography Awards in April 2023, the winner Eldagsen refused his award after revealing that his creation was made using AI. Organizers of the award said that Eldagsen had misled them about the extent of AI that would be involved~\cite{bbc}.
In this study, our human evaluation results indicate that the state-of-the-art (SOTA) AI model is able to deceive the human eye to a significant degree (38.7\%).
Moreover, our exploration shows that it is no longer reliable to judge whether an image is real based solely on image quality. 
Instead, people need to consider factors such as over-smoothing portrait faces, coherence, and consistency between objects, and physical laws in the image, which makes the distinguishing process much harder and time-consuming (about 18 seconds for each image in this study).
% whether the portrait is too smooth, the coherence and consistency between objects, and whether there are any violations of physical laws in the image.

% However, this does not necessarily mean that AI can stably generate high-quality images which can deceive the human eye. In fact, creating such high-quality images requires a certain level of skill and a lot of experiments. Nevertheless, AI does have the capability to produce high quality images to deceive human perception.
From another aspect, current AI still can not \textbf{consistently} deceive the human eye.
AI-generated images still have certain defeats which could be used by humans to distinguish fake images. 
Besides, creating such high-quality images requires prompt engineering skills and numerous experiments. 
% Nevertheless, AI does have the capability to produce high-quality images that can deceive human perception.
Even though, a few finely adjusted AI images with misleading information can convey wrong ideas and cause enormous damage.

\paragraph{What the current state-of-the-art image generation model can do and can not do?}
% The current state-of-the-art image generation model has the ability to produce photorealistic images that are practically indistinguishable from real photographs based on a sentence description or an image, as shown in Fig.~\ref{identify}. This description can be as simple or as complex as needed, and may include details such as colors, textures, and lighting. The potential applications of AIGC are numerous and diverse. For instance, it can be used to generate images for advertising campaigns, product catalogs, and fashion magazines. It can also be utilized in the film industry to create realistic special effects or even entire scenes. Furthermore, AIGC can be implemented in the gaming industry to produce immersive and lifelike game worlds.
Given suitable prompts, the SOTA image generation model can produce photo-realistic images that are indistinguishable from real photographs, as shown in Fig.~\ref{identify}. 
The prompt can have different formats (e.g., text, image) and arbitrary complexity, including details such as colors, textures, and lighting.
% be as simple or as complex as needed and may include details such as colors, textures, and lighting. 
% The potential applications of AIGC are numerous and diverse. 
There are lots of potential applications for image generation.
For instance, AIGC can be used to generate images for advertising campaigns, product catalogs, and fashion magazines. 
Since it can easily be controlled by text, AIGC can also be utilized in the film industry to create realistic special effects or even entire scenes, at an extremely low cost.
Furthermore, AIGC can be implemented in the gaming industry to produce immersive and lifelike game worlds.

% Although the current state-of-the-art image generation model has impressive image generation capabilities, it currently faces several limitations and drawbacks, as shown in Fig.~\ref{AIGC defects}. One of the most significant challenges is generating images of multiple people in a single scene. The model struggles to accurately represent complex social dynamics and interactions between individuals.
% Furthermore, the current state-of-the-art image generation model has difficulty generating realistic human hand gestures and positions, which are crucial for many applications such as sign language recognition and virtual reality. The model also struggles to generate complex textual symbols in the images.
% In addition, the current state-of-the-art image generation model can produce images with strange details, blurriness, and unrealistic physical phenomena like lighting issues. These issues limit the model's ability to generate images with high accuracy and fidelity to real-world scenes.
% Overall, while the current state-of-the-art image generation model has shown remarkable capabilities in generating images from text descriptions, it still faces significant challenges that need to be addressed for it to achieve even greater success in the field of image generation.

Although generative AI has impressive image generation capabilities, it currently faces several limitations and challenges, as shown in Fig.~\ref{AIGC defects}. 
% \whlzy{before not mentioned}
One of the most significant challenges is generating images of multiple people with intricate details in a single scene. 
% The model struggles to accurately represent complex body interactions and social relationships between individuals. 
Users can easily infer the authenticity of an image from details.
%Done by remove and add a new sentence \xihui{Can we add some failure cases corresponding to it? We don't have this type of examples in the paper.}
Furthermore, the current model has difficulty generating realistic human hand gestures and positions, which are crucial for many applications such as sign language recognition and virtual reality. 
% The model also struggles to generate complex textual symbols in the images.
In addition, the current state-of-the-art image generation model can produce images with strange details, blurriness, and unrealistic physical phenomena such as lighting issues. These issues limit the model's ability to generate images with high accuracy and fidelity to real-world scenes.
Overall, while the SOTA image generation model has shown remarkable capabilities, it still faces significant challenges that need to be addressed for it to achieve even greater success in the field of image generation.

\subsection{Broader Impact}

\paragraph{Societal risks.}
% As AI-generated content (AIGC) continues to be promoted in various fields, concerns about its societal use have become increasingly prominent. These concerns involve various issues such as bias, ethics, and the impact of AIGC on various stakeholders. As we have demonstrated in this article, it is already becoming difficult for humans to distinguish between AI-generated images and real images. Therefore, the current state-of-the-art image generation model may produce contents that contradict or even absurdly violate reality, posing a serious threat to factual information on the Internet. Photos may become increasingly difficult to use as evidence in the future, and even serious public opinion effects may result. For example, there were many AI-generated images of Trump being arrested on Twitter recently. Such content may be used to spread false information, incite violence, or harm individuals or organizations. In addition to the potential for false information and confusion of authenticity, AIGC may also bring many other problems. AIGC can be used to create virtual characters that can look very realistic. These virtual characters may be used for malicious purposes such as online fraud, scams, or harassment. For example, a virtual character may be used to impersonate a real person in order to obtain their personal or sensitive information. AIGC may also be used for political propaganda or other malicious purposes. For instance, false speeches or statements by political figures may be produced using AIGC, leading to public misinformation or social chaos.
As AIGC continues to be promoted in various fields, concerns about its societal use have become increasingly prominent. 
These concerns involve various issues such as bias and ethics.
As we have demonstrated, it is getting more and more difficult for humans to distinguish between AI-generated images and real images. 
Therefore, AI models may produce content that contradicts or even absurdly violates reality, posing a serious threat to factual information. 
Photos may then become increasingly difficult to use as evidence in the future, and even serious public opinion effects may result. 
For example, there were many AI-generated images of Trump being arrested on Twitter recently~\cite{bbc2}. 
Such content may be used to spread false information, incite violence, or harm individuals or organizations. 
Besides, AIGC can be used to create realistic virtual characters, which may be used for malicious purposes such as online fraud, scams, or harassment. 

% In addition to the potential for false information and confusion of authenticity, AIGC may also bring many other problems. 
% AIGC can be used to create virtual characters that can look very realistic. These virtual characters may be used for malicious purposes such as online fraud, scams, or harassment. 
% For example, a virtual character may be used to impersonate a real person in order to obtain their personal or sensitive information. AIGC may also be used for political propaganda or other malicious purposes. 
% For instance, false speeches or statements by political figures may be produced using AIGC, leading to public misinformation or social chaos. 

% It is crucial that researchers and practitioners in the field of AIGC work towards developing strategies to mitigate these potential negative impacts. This includes developing ways to identify AIGC, establishing guidelines for ethical use of AIGC, and promoting awareness among the public about the existence and potential impact of AIGC. Only by working together can we ensure that the benefits of AIGC are fully realized while also minimizing its negative consequences.
It is crucial for researchers and practitioners in the field of AIGC to develop strategies to mitigate potential negative impacts. This includes developing methods to identify AI-generated images, establishing guidelines for their ethical use, and raising public awareness about their existence and potential impact. Only by working together can we ensure that the benefits of AIGC are fully realized while minimizing its negative consequences.

\paragraph{Positive impacts.}
% On the other hand, given that AI has shown remarkable performance in creating works of art and photography, it is expected to have a significant impact on artists and photographers in the real world. People can obtain a large number of desired works or photos at a lower cost. This will greatly compress the space of artists and photographers. In this era of fast-food images, where should the new generation of artists and photographers go? However, AI can only generate soulless works, lacking the creativity, imagination, and emotion possessed by human artists and photographers. Even the most advanced AI technology cannot replace the creativity and individuality of human artists and photographers. Therefore, although the emergence of AI has indeed brought new challenges and changes to the fields of art and photography, the value and existence of human artists and photographers are still preserved. At the same time, the emergence of AI also provides new opportunities for artists and photographers. They can use AI technology to create new works of art or design new photos. In addition, AI technology can also be used to improve and optimize existing works and photos, thereby improving the quality and value of works of art and photos. Therefore, artists and photographers need to constantly learn and explore AI technology to adapt to new market demands and technological changes.
Given that AI has shown remarkable performance in creating works of art and photography, it is expected to have a significant impact on artists and photographers in the real world. 
People can obtain a large number of desired works or photos at a lower cost, which could compress the market for artists and photographers. 
In this era of fast-food images, where should the new generation of artists and photographers go~\cite{bbc3}? 
However, AI can only generate soulless works, lacking the creativity, imagination, and emotion possessed by human artists and photographers~\cite{Yanru-2022-HumanAI}. 
Even the most advanced AI technology cannot replace the creativity and individuality of human artists and photographers. 
Therefore, although the emergence of AI has indeed brought new challenges and changes to the fields of art and photography, human artists and photographers are still highly valued. 

% At the same time, the emergence of AI also provides new opportunities for artists, photographers, designers and users. 
% They can use AI technology to create new visual creations, such as digital arts, photos or logos, reducing the time and cost associated with traditional methods of image creation.
% AI technology can generate novel and unique images that may not have been created otherwise, leading to new ideas and inspiration for designers and artists.
% AI technology can also be used to improve and optimize existing works and photos, thereby enhancing the quality and value of works of art and photos. 
% Users can create personalized images based on specific preferences, leading to a more engaging and customized experience.
% Therefore, artists, photographers, designers and users need to constantly learn and explore AI technology to adapt to new market demands and technological changes.

%Not all AI technologies are malicious.
The emergence of AI technology presents various new opportunities for artists, designers, and users. 
One of the most significant benefits is the ability to create new and innovative visual works, such as digital art and logos, while reducing the time and cost associated with traditional image creation methods. 
AI technology allows people to generate unique and novel images that might not have been possible otherwise, leading to new ideas and inspiration. 
Moreover, AI technology can help optimize existing works of art and photos, leading to improved quality and value. 
For instance, AI can be used to enhance or restore old or damaged images to their original state~\cite{Ziyu-2020-oldphoto}, which can be particularly useful in restoring historic photographs or artworks~\cite{bbc4}. 
AIGC also provides users a more personalized experience by creating images tailored to their personal preferences~\cite{Rinon-2022-textinvision, Nataniel-2022-dreambooth}. 
This customization can lead to more engaging and immersive experiences for users. 
% As the market demands and technological changes continue to evolve, artists, photographers, designers, and users need to keep pace with the latest AI developments. They must continually learn and explore AI technology to stay competitive and relevant in their respective fields. 

% In conclusion, AI technology offers numerous opportunities for creativity, innovation, and customization in the art and design industry, and it is crucial for professionals and users to embrace and leverage these opportunities to remain successful.
% AIGC also can open up new career paths and opportunities for professionals seeking to advance their careers in the rapidly growing field of AI and machine learning.

\paragraph{Academic impacts.}
% 1. Need Identify AI
% 2. User Privacy
% 3. A human perception test for AIGC
% 4. AIGC can be used as training data 
% We conducted a qualitative and quantitative evaluation of the most advanced image generation model from the perspective of whether humans can discern whether an image is generated by AI. Based on our evaluation, we have summarized some academic issues that need to be addressed:
In this study, we conduct a quantitative human evaluation of whether the most advanced AI model can deceive the human eye. 
% Based on our evaluation, we have summarized several academic issues that need to be addressed:
Results indicate several academic directions that could be explored in the future:

\noindent{\textbf{$\bullet$}}
Since people cannot discern the authenticity of images, a natural question arises: \textit{Can AI distinguish whether an image is generated by AI?} 
Exploring how to use AI to detect AI-generated images is a problem that could be studied ~\cite{Sheng-2020-GeneratedFake}. 
Establishing a detection system to recognize AIGC will greatly ensure the security of society and the credibility of images.

\noindent{\textbf{$\bullet$}}
Even the most advanced image generation model still cannot guarantee the stable generation of high-quality images. 
At the same time, as shown in Fig.~\ref{AIGC defects} and Tab.~\ref{judgement}, AI-generated images often have certain defects. 
Our failure case analysis will inspire researchers to design better image generation models. 
Exploring how to solve these AIGC defects is an important future research direction.

\noindent{\textbf{$\bullet$}}
In the real world, it is difficult to obtain comprehensive and diverse data, leading to the famous problem of data imbalance~\cite{Justin-2019-imbalance}. 
Using imbalanced data will result in various issues such as the long-tail problem~\cite{Yifan-2021-longtail} and bias problem~\cite{Ninareh-2022-Bias}. 
Since the current state-of-the-art image generation model can already produce high-quality data, exploring how to use the image generation model to solve these problems and test the current model's robustness and bias is a problem that could be studied.

\subsection{Conclusion}
% In this paper, we conclude that the current state-of-the-art image generation model can indeed significantly deceive human perception: a high-quality AI-generated image can be comparable to a real photograph.
% We have focused on the surprising things that the current state-of-the-art image generation model can do and can not do, but we do not address the core questions of why and how it achieves such remarkable intelligence and the most important problems of how to ensure the security of AIGC and credibility of images.
In this paper, we conclude that the current SOTA image generation model can indeed significantly deceive human perception: high-quality AI-generated images can be comparable to real photographs. 
We have focused on the surprising abilities of the current SOTA image generation model, but we have not addressed the core questions of why and how it achieves such remarkable intelligence, nor the most important issues of how to ensure the security and credibility of AIGC images.
% Overall, the progress of the current SOTA image generation model is indeed astonishing. 
% However, it also poses a significant challenge for researchers to develop secure and reliable AIGC systems that can be trusted for various real-world applications. 
It is a significant challenge for researchers to develop secure and reliable AIGC systems that can be trusted for various real-world applications, and ensure the responsible and ethical use of AIGC technology in the future.
% Therefore, more research and development efforts are needed to tackle these challenges and ensure the responsible and ethical use of AIGC technology in the future.
% Overall, elucidating the nature and mechanisms of AI systems such as GPT-4 is a formidable challenge that has suddenly become important and urgent.
It is time to prioritize responsible development and the use of generative AI to ensure a positive impact on society.

%But solving the security and privacy problems of AIGC is a formidable challenge that has suddenly become important and urgent.
% Overall, the progress of the current ate-of-the-art image generation model is indeed astonishing. 
% But it also poses a significant challenge to the researchers to develop secure and reliable AIGC systems that can be trusted for various real-world applications. 
% Therefore, more research and development efforts are needed to tackle these challenges and to ensure the responsible and ethical use of AIGC technology in the future.

% In this paper, we report on our investigation of the current state-of-the-art image generation model. We contend that the current state-of-the-art image generation model can indeed significantly deceive human perception that exhibit more general intelligence than previous AI models, although its generation quality is not yet very stable. Our results also reveals that an individual’s personal background does not significantly impact their ability to perceive AI-generated images. In our exploration of the state-of-the-art image generation model, we put special emphasis on discovering its defects, and we discuss the challenges ahead for advancing towards more comprehensive versions of image generation model. Finally, we reflect on the societal impacts of the recent technological leap and suggest potential directions for future research.




==> content_version1/7_checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> content_version2/8_checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{}
\end{enumerate}

\end{enumerate}

==> extra_pkgs.tex <==
\usepackage[ruled]{algorithm2e}
\usepackage{hyperref}
\usepackage{microtype}
\usepackage{pifont}
\usepackage{xcolor}
\usepackage{xurl}
% Figures and Tables
\usepackage{graphicx}
\usepackage{booktabs, multirow}
% Monospaced Code Blocks
\usepackage{listings}
% Math Packages
\usepackage{amsmath, amsfonts, amsthm}
\usepackage{nicefrac}
\usepackage{bbding}

\lstset{
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\ttfamily,            % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  columns=fullflexible,            % reduce the column spacing
  commentstyle=\color{gray},       % comment style
  deletekeywords={},               % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=none,                      % adds no frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=C++,                    % the language of the code
  morekeywords={},                 % if you want to add more keywords to the set
  numbers=none,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\color{black},       % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{red},         % string literal style
  tabsize=4,                       % sets default tabsize to 4 spaces
}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{remark}{Remark}
\newtheorem*{example}{Example}


==> figure/distribution_for_all_categories.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figure/distribution_for_all_categories_fig.pdf}
    % \vspace{-0.1cm}
    \caption{
        \textbf{Overall score distributions.}
    }
    % \vspace{-0.2cm}
    \label{distribution for all categories}
\end{figure*}

==> table/descri.tex <==
\begin{table}[]
\begin{tabular}{ll}
Dataset Name        & Dataset Description                            \\
CC3M-Train          & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
StyleGAN3-Train     & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
SD-V2.1-dpms-25     & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
SD-V1.5Real-dpms-25 & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
IF-V1.0-dpms++-25   & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
StyleGAN3           & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
ImageNet-Test       & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
CelebA-HQ-Train     & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
CC3M-Val            & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
SD-V2.1-dpms-25     & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
SD-V1.5-dpms-25     & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
SD-V1.5Real-dpms-25 & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
IF-V1.0-dpms++-10   & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
IF-V1.0-dpms++-25   & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
IF-V1.0-dpms++-50   & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
IF-V1.0-ddim-50     & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
IF-V1.0-ddpms-50    & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
Cogview2            & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
Midjourney          & Stable Diffusion v2.1 with DPM-Solver 25 steps \\
StyleGan3           & Stable Diffusion v2.1 with DPM-Solver 25 steps
\end{tabular}
\end{table}

==> table/metric_aigc.tex <==
\begin{table*}[t]
\centering
\caption{Performance of the people which have played with the AIGC and have not played with the AIGC.}

\resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Metric} & \multicolumn{9}{c}{Category}                                              \\
                        & all & humans & landscape & man & woman & record & plant & animal & object \\ \midrule[1.2pt]
\textbf{Accuracy}  &     &        &           &     &       &        &       &        &        \\
\textbf{Precision} &     &        &           &     &       &        &       &        &        \\
\textbf{Recall}    &     &        &           &     &       &        &       &        &        \\
\textbf{False Omission Rate}    &     &        &           &     &       &        &       &        &        \\
% \textbf{$F_1$ Score}   &     &        &           &     &       &        &       &        &        \\
\bottomrule[1.2pt]
\end{tabular}
}

\label{metric_aigc}
\end{table*}

==> table/metric_man_woman.tex <==
\begin{table*}[!t]
\centering
\caption{Performance of man and woman.}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Metric} & \multicolumn{9}{c}{Category}                                              \\
                        & all & humans & landscape & man & woman & record & plant & animal & object \\ \midrule[1.2pt]
\textbf{Accuracy}  &     &        &           &     &       &        &       &        &        \\
\textbf{Precision} &     &        &           &     &       &        &       &        &        \\
\textbf{Recall}    &     &        &           &     &       &        &       &        &        \\
\textbf{False Omission Rate}    &     &        &           &     &       &        &       &        &        \\
% \textbf{$F_1$ Score}   &     &        &           &     &       &        &       &        &        \\
\bottomrule[1.2pt]
\end{tabular}
}

\label{metric_man_woman}
\end{table*}
